On the Influence of Masking Policies in Intermediate Pre-training

Current NLP models are predominantly trained through a two-stage "pre-train then fine-tune" pipeline. Prior work has shown that inserting an intermediate pre-training stage, using heuristic masking policies for masked language modeling (MLM), can significantly improve final performance. However, it is still unclear (1) in what cases such intermediate pre-training is helpful, (2) whether hand-crafted heuristic objectives are optimal for a given task, and (3) whether a masking policy designed for one task is generalizable beyond that task. In this paper, we perform a large-scale empirical study to investigate the effect of various masking policies in intermediate pre-training with nine selected tasks across three categories. Crucially, we introduce methods to automate the discovery of optimal masking policies via direct supervision or meta-learning. We conclude that the success of intermediate pre-training is dependent on appropriate pre-train corpus, selection of output format (i.e., masked spans or full sentence), and clear understanding of the role that MLM plays for the downstream task. In addition, we find our learned masking policies outperform the heuristic of masking named entities on TriviaQA, and policies learned from one task can positively transfer to other tasks in certain cases, inviting future research in this direction.

==> archive/4_deprecated_experiment.tex <==
\section{Results and Discussion}
\label{sec:exp-results}
We list the results for closed-book QA tasks in Table \ref{tab:cbqa}, knowledge-intensive language tasks in Table \ref{tab:kilt} and summarization tasks in Table \ref{tab:summarization-simplified}.

\subsection{Closed-book QA} 

First, we observe performance gains with further pre-training with random masks on BART-base. This may be due to the common observation that language models tend to improve with further pre-training even after validation perplexity have plateaued \cite{conneau2019unsupervised}. Moreover, the Wikipedia corpus is more closely related to the three closed-book QA tasks than BART's original pre-training set\footnote{BART was originally pre-trained on a combination of news, books, stories, and web text, the same as in RoBERTa \cite{liu2019roberta}.}.

In addition, SSM does indeed serve as a strong heuristic objective, as  \citet{roberts2020much} found. Our absolute performance gain is less significant than theirs; we hypothesize this is due to the smaller size of our models (BART-base has 140M parameters, compared to 11B in T5-11B).
\input{tables/closed-book}
As for learned masking policies, the effect is most significant on TriviaQA. Our supervised policy achieves $24.71\%_{\pm.21}$, which outperforms SSM heuristic ($23.62\%_{\pm.29}$), with $p=0.03$. Our meta-learned policy achieves $23.88\%_{\pm.04}$ which outperforms the original objective ($22.91\%_{\pm.16}$), with $p=0.03$, and becomes comparable with SSM. These results demonstrate that the learned policies, either supervised or meta-learned, learns meaningful information from the downstream tasks and helps to encode task-specific knowledge during intermediate pre-training.

The patterns for WQ and NQ results are less clear. On WQ, supervised policies and SSM appear to be the best, while the differences between different methods are not statistically significant. We note that the performance on WQ is unstable, and we conjecture the reason to be its relatively small size (Train 3417, Dev 361, Test 2032). Similarly, performances are close for each method on NQ. We discuss the factors behind this phenomenon in Appendix \ref{app:nq}. 

\subsection{Knowledge-Intensive Language Tasks}

% On knowledge-intensive language tasks we have the following observations. 
By comparing the first three rows in Table \ref{tab:kilt}, we see that BART-Base and +Orig are better for WoW, while +Rand is better for AY2 and ZSRE. 
Note that the outputs of WoW is coherent sentences, while the output of AY2 and ZSRE are short spans. 
Also, the major difference between +Orig and +Rand is whether the full sequence or the masked tokens are generated. 
We conclude that the tasks that requires generating short spans are more likely to benefit from pre-train objectives that generates short spans (+Rand); and similarly, tasks that generates long, coherent sentences are likely to benefit from a similar pre-train task (+Orig).
This conclusion is further supported by the results of learned policies, where the best performing model for AY2 and ZSRE both comes from pre-training objectives that generates short spans, while WoW has the best performance when using BART-Base, Orig and meta-learned policy, all of which are from pre-train objective that generates long sentences. 

We notice that the supervised policy learned from ZSRE outperforms +Rand baseline, but does not outperform +SSM heuristic. This suggest that the learned policy has learned meaningful signals, but may suffer from over-fitting, as the train-test distribution is drastically different for ZSRE dataset. SSM is agnostic to such train-test discrepancy and thus achieves the strongest performance.
% The supervised policy learned from the train set may focus on the information related to the train relations, while not generalizing to test relations.

\subsection{Summarization}
\input{tables/kilt}

For summarization tasks we observe performance deterioration with intermediate pre-training, regardless of what the masking policy is used. We conjecture that this is due to our choice of pre-train \textit{corpus} or \textit{scale}. Both CNN/DM and XSum falls into the news domain, so that pre-training on Wikipedia may leads to domain shift that worsens the performance. Also, for \{+Orig,+Rand,+SSM\} checkpoints, we uses a smaller sequence length (128) than the original BART (512), which may further hurt performance. 
Due to these concerns, we have shaded the row of BART-base in Table \ref{tab:summarization-simplified} to help focus the comparison on the remaining methods. 

Secondly, we found that meta-learned policies do not bring significant improvements. Note that we set $\mathbf{c}=\mathbf{s}$ as an approximation during meta-learning for summarization tasks. The results suggest the proposed meta-learning methods might not be suitable for tasks that are not in $(\mathbf{c}, \mathbf{s}, \mathbf{t})$ format.

Some other observations include: (1) +SSM outperforms +Rand, suggesting that named entities play an important role in summarization. (2) Masking random sentences in the instance (+MaskRandomSentence) achieves the best performance. 
\input{tables/summarization_simplified}

\subsection{Discussion}
\label{sec:discussion}
Based on our observations from previous experiments, we revisit the question raised in the introduction, and offer suggestions to NLP researchers and practitioners who wish to improve downstream performance via intermediate pre-training.

The first question is \textbf{whether to conduct intermediate pre-training or not}. Prior work has shown that continue pre-training with in-domain corpora helps to improve downstream performance \cite{gururangan-etal-2020-dont}. Our experiments on summarization suggest pre-training on an \textit{out-of-domain corpus} with promising heuristics or masking policies, or with \textit{smaller pre-training scale} (batch size, sequence length), would hurt final performance. Lack of in-domain corpus or sufficient computation resources may lead to in-successful intermediate pre-training.

The second question is \textbf{among heuristic policies, which one should be used during intermediate pre-training}. 
If there is heuristic masking policies that resembles the downstream task, typically this would bring improvements, as demonstrated with SSM and random sentence masking. 
If the heuristic is less clear, using random masking on in-domain corpus would also be helpful, as demonstrated with closed-book QA tasks.
If choosing to use random masking, we recommend to decide whether to generate full sequence (+Orig) or only masked tokens (+Rand) based on the task output length. If the downstream tasks requires generating coherent sentence (\textit{e.g.}, dialogue, summarization), generating full sequence is more helpful; otherwise (\textit{e.g.}, closed-book QA, entity linking), generating masked tokens is more helpful. 

The third question is in \textbf{whether learned policies can be better than heuristics}. 
Our answer is that this depends on the downstream tasks. 
For both of our proposed methods, learning a masking policy requires supervision from $(\mathbf{c}, \mathbf{s}, \mathbf{t})$ examples. In this case, closed-book QA and knowledge-intensive tasks are more likely to benefit from learned policies, while summarization will not since it does not have a context paragraph by design. 
We recommend to use learned policies in two cases: 
(1) $(\mathbf{c}, \mathbf{s}, \mathbf{t})$ examples are abundant, train/test distributions are consistent, and the heuristic does not perfectly resemble the task. In our experiments, TriviaQA has these characteristics and benefits from learned policies most.
(2) For tasks whose heuristic masking policy is not intuitive (e.g., WoW), meta-learned masking policy is worth trying.
We also highlight that using learned policies has potential risks of over-fitting to training instances, or suffering from high instability in meta-learning. Future work may investigate these issues and improve our proposed methods.

==> archive/4_experiment.tex <==

\section{Experiments}

\subsection{Experiment Setup}
\paragraph{Datasets.}
Following \citet{roberts2020much}, we experiment with three open-domain QA benchmarks: Natural Questions (NQ), WebQuestions (WQ, \citealt{berant-etal-2013-semantic}) and \mbox{TriviaQA} (TQA) in the closed-book setting. We use the train/dev/test splits that are consistent with \citet{lee-etal-2019-latent} and \citet{karpukhin-etal-2020-dense}. 

\paragraph{Baselines.}
We report closed-book QA performance when fine-tuned on the following different checkpoints: (1) Publicly released BART-base model (BART); (2) Intermediate pre-training by masking $15\%$ randomly selected tokens (+Random); (3) Intermediate pre-training with salient span masking\footnote{The named entity tags are obtained with \href{https://spacy.io/}{spaCy}.} \cite{roberts2020much, guu2020realm} (+SSM). Alongside, we report performance when applying our own learned policy to intermediate pre-training (+Learned). To ensure fair comparison, all intermediate pre-training is done with input sequence length of 128, batch size of 2048, learning rate of $0.0001$, and a total number of $100,000$ updates, using Wikipedia snapshot from December 20, 2018\footnote{The snapshot is available at \url{https://archive.org/download/enwiki-20181220}. Wikipedia is licensed under \href{https://creativecommons.org/licenses/by-sa/3.0/}{CC BY-SA 3.0}.}. We use the linear learning rate warmup schedule for the first $6\%$ of steps, and linear decay for the remaining steps.

\paragraph{Fine-tuning.}
We take each checkpoint from the baselines, along with the checkpoint using our own learned policy, and fine-tune it on the three closed-book QA datasets separately. We use Adam \cite{Kingma2015AdamAM} optimizer for BART-base experiments, and Adafactor~\cite{pmlr-v80-shazeer18a} for BART-large. For hyperparameter settings, please refer to Appendix \ref{app:hps}. We report the average and standard deviation of performance using three random seeds. We report exact match after standard normalization \cite{rajpurkar-etal-2016-squad}.


\subsection{Results and Discussion} 
% We list experimental results in Table \ref{tab:closed-book-tqa}. 

\paragraph{TriviaQA Results.} We first experiment with TriviaQA since TriviaQA benefits most from SSM in \cite{roberts2020much}. That is, we learn a masking policy from TriviaQA, plug the policy to intermediate pre-training, and then fine-tune on TriviaQA. We list the performance in Table \ref{tab:closed-book-tqa}. 
From the table, we make multiple key observations.

First of all, we observe performance gain with further pre-training with random masks on BART-base. This may be due to the common observation that language models tend to improve with further pretraining even after validation perplexity have plateaued \cite{conneau2019unsupervised}, or that Wikipedia corpus is more closely related to the three closed-book QA tasks\footnote{BART was originally pre-trained on a combination of news, books, stories, and web text, the same as in RoBERTa \cite{liu2019roberta}.}.

In addition, SSM does indeed serve as a strong heuristic objective as described in \citet{roberts2020much}. Our absolute performance gain is less significant, with $0.8\%$ improvement on BART-base and $2.0\%$ improvement on BART-large. We hypothesize this is due to the smaller size of BART models (140M/406M parameters for BART-base/large, compared to 11B in T5-11B).

As for our proposed approach, the masking policy learned on TriviaQA achieves the strongest performance, surpassing SSM in both BART-base and BART-large experiments. This demonstrates that the our method is effective for TriviaQA. Notably, pre-training BART-base with the learned policy outperforms original BART-large model (EM=$24.71\%$ vs EM=$24.28\%$, respectively), effectively saving 260M parameters in the LM. 

% \input{tables/cbqa-results-tqa-only}

\paragraph{Extending to More Datasets.} We further extend our experiments to policies learned from different anchor tasks and fine-tune across all three downstream task separately. We list the full results in Table \ref{tab:closed-book}. We observe that the learned masking policy ``transfers'' in some (but not all) cases: The Learned(NQ, Top5) policy helps to achieve $23.73\%_{(\pm.21)}$ EM on TriviaQA, which is on par with SSM; The Learned(TQA, Top5) transfers to Web Questions, also achieving results on par with SSM. This observation suggests that the learned policy may capture transferable meta-knowledge on ``what information is important for closed-book QA'', though such improvement is not consistent across all settings.

\paragraph{Discussion on NQ.} In Table \ref{tab:closed-book} we also observe that performances on NQ are close for all BART-base models; therefore it is hard to rank all compared methods. We argue that multiple factors leads to this phenomenon, including dataset characteristics and evaluation protocol.
Specifically, NQ may not be an ideal testbed for our study due to three reasons. 

Firstly, intermediate pre-training in general might not be as beneficial for this particular task. For instance,
\citet{roberts2020much} reports only 2\% EM gain on NQ using T5-11B. In our experiments, we use significantly smaller pre-trained models (BART-base/large), so the effect brought by intermediate pre-training will be even smaller. 
In our case we believe the effect is hidden in the variance brought by random seeds. 

Secondly, performance on NQ may not represent the real implicit knowledge capacity of a LM. For reference, we observe a 20\% dev set EM when fine-tuning a randomly initialized BART-base model on NQ. The general pre-training stage brings merely 4-5\% EM improvement, and therefore the improvement brought by intermediate pre-training can be marginal. 

And finally, evaluation based on exact match may substantially underestimate the model capability, as suggested in \cite{roberts2020much}.


% \input{tables/case_study}
% \input{tables/cbqa-results}

\subsection{Case Study of the Learned Policy} 
We use the policy trained on TriviaQA and provide its prediction on TriviaQA dev set context paragraphs in Table \ref{tab:example}. We observe that the policy is masking important spans within the context paragraph as expected. One limitation is that the start position and end position are determined independently, so that ``Chadwick School and later attended the University of California'' becomes an candidate answer span because the start position logit for ``Chadwick'' is large, and the end position logit for ``California'' is large. Ideally ``Chadwick School'' and ``University of California'' should be masked separately. Similar problem holds for machine reading comprehension models, and this is a limitation of our current approach. 
% In the future, we may consider combining the predictions with constituency parsing results to ensure a constituent is masked.

% \subsection{Discussion}

==> figures/2d_visualization.tex <==
\begin{figure}
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/2d-sup.pdf}
  \caption{Supervised Policies}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=\textwidth]{figures/2d-meta.pdf}
  \caption{Meta-learned Policies}
  \label{fig:sub2}
\end{subfigure}
\vspace{-0.3cm}
\caption{\textbf{2D Visualization of learned policies.} Policies learned from TQA and ZSRE are closest to SSM. Policies learned from tasks that test a model's implicit knowledge capacity are close to each other. These observations align with the nature of the tasks.}
\label{fig:2d}
\vspace{-0.5cm}
\end{figure}

==> sections/0_abs.tex <==
% Intermediate pre-training is a phase between general pre-training and task-specific fine-tuning that aims to adjust the language model to target domains or tasks. 
% Prior work has shown that adopting heuristic objectives that resemble downstream tasks during intermediate pre-training improves final performance. 
Current NLP models are predominantly trained through a pretrain-then-finetune pipeline, where models are first pretrained on a large text corpus with a masked-language-modelling (MLM) objective, then finetuned on the downstream task.
Prior work has shown that inserting %shown that continuing to pre-train language models, in 
an \textit{intermediate} pre-training phase, with heuristic MLM objectives that resemble downstream tasks, can significantly improve final performance.
However, it is still unclear (1) \textit{in what cases} such intermediate pre-training is helpful, (2) whether hand-crafted heuristic objectives are \textit{optimal} for a given task, and (3) whether a MLM policy designed for one task is \textit{generalizable} beyond that task. 
In this paper, we perform a large-scale empirical study to investigate the effect of various MLM policies in intermediate pre-training. Crucially, we introduce methods to \textit{automate} discovery of optimal MLM policies, by \textit{learning} a masking model through either direct supervision or meta-learning on the downstream task. 
% We continue to pre-train an off-the-shelf language model with heuristic, directly supervised, or meta-learned MLM policies, then fine-tune the resulting models on eight selected tasks across three categories (closed-book QA, knowledge-intensive language tasks, and abstractive summarization). 
We investigate the effects of using heuristic, directly supervised, and meta-learned MLM policies for intermediate pretraining, on eight selected tasks across three categories (closed-book QA, knowledge-intensive language tasks, and abstractive summarization).
% \qinyuan{trying my best but we still need a better ending for the abstract.}
% We provide detailed analysis on the experimental results and masking policies used, trying to answer the research questions we raised in the beginning.
Most notably, we show that learned masking policies outperform the heuristic of masking named entities on TriviaQA, and masking policies learned on one task can positively transfer to other tasks in certain cases.
% For entity-centric tasks such as closed-book QA, we observe that masking and recovering named entities consistently improves performance, and a learned policy further outperforms this heuristic on TriviaQA. 
% Overall, our study suggests that the optimal masking policy depends on the downstream task itself. Additional factors such as output length, task format, and availability of resources should be taken into consideration as well.

% Closed-book question-answering (QA) is a challenging task that requires a model to directly answer questions without access to external knowledge.
% It has been shown that directly fine-tuning pre-trained language models with (question, answer) examples yields surprisingly competitive performance,
% which is further improved upon through adding an intermediate pre-training stage between general pre-training and fine-tuning.
% Prior work used a heuristic during this intermediate stage, whereby named entities and dates are masked, and the model is trained to recover these tokens. 
% In this paper, we aim to \textit{learn} the optimal masking strategy for the intermediate pre-training stage. Toward this goal, we experiment with two different methods: (1) a supervised policy; (2) a meta-learned policy. We extensively experiment with different policies learned with these approaches.

% Pre-training objectives (\textit{e.g.}, masked language modeling) are mostly heuristic and based on random sampling. In this paper, towards to goal of packing more knowledge into the pre-trained model parameters, we investigate several masking strategies during pre-training: 
% (1) A meta-learned policy that enables answering a query well after pre-trained on relevant context;
% (2) A extractive policy that learns to extract answer span frrom (context, answer) examples, without the query;
% (3) Heuristic masking strategies such as salient span masking, span corruption, and denoising.
% We deploy these strategies into intermediate pre-training (as opposed to general pre-training), and test the implicit knowledge capacity of the pre-trained models on a wide range of knowledge-intensive tasks.

==> sections/1_introduction.tex <==
\section{Introduction}

% \blfootnote{$^\dagger$Work partially done while interning at Facebook AI.}
% \blfootnote{$^\ddagger$Work partially done while working at Facebook AI.}


Large, neural language models (LMs) pre-trained with masked language modeling \cite{devlin-etal-2019-bert,raffel2019exploring} have achieved impressive results over a variety of NLP tasks.\blfootnote{$^\dagger$Work partially done while interning at Facebook AI.}\blfootnote{$^\ddagger$Work partially done while working at Facebook AI.}
Studies show that an additional intermediate pre-training stage between general pre-training and task-specific fine-tuning further improves downstream performance (Fig. \ref{fig:intro}).
For example, salient span masking (SSM), the pre-training objective of recovering masked named entities or dates \cite{guu2020realm}, significantly improves performance of closed-book QA \cite{roberts2020much}, a task that requires a model to answer factoid questions without access to external knowledge. 
% However, it is yet unclear whether these masking heuristics are optimal, or whether they generalize to NLP tasks with different formats and goals.
However, there is a lack of systematic study on how intermediate pre-training works, whether the heuristic masking policies like SSM are near-optimal, or whether they generalize to different NLP tasks. Additionally, it is unclear that for tasks other than closed-book QA, whether intermediate pre-training is helpful, or what masking strategy should be adopted. 

\input{figures/intro}

In this paper, we offer a large-scale, systematic study on the effects and transferability of masking strategies during intermediate pre-training. 
% Specifically, we take an off-the-shelf pre-trained language model as initialization and further adopt a two-stage pipeline of intermediate pre-training and downstream task fine-tuning.
% \qinyuan{will rewrite so this part is consistent with the new section 5}
We measure such influence by deploying different masking strategies during intermediate pre-training, while carefully controlling all other aspects (\S\ref{sec:analysis-setup}). Through these experiments, we aim to answer the following questions:
\begin{itemize}[leftmargin=*]
    \item \textbf{Q1.} Is intermediate pre-training suitable for different NLP tasks? Should we conduct it or not?
    % Are heuristic masking policies optimal? Can we learn a masking policy from the downstream task to better guide its own intermediate pre-training? 
    \item \textbf{Q2.} Given several heuristic masking policies, how to choose the best one?
    \item \textbf{Q3.} Can we learn a masking policy to better capture the characteristics of downstream tasks?
    \item \textbf{Q4.} Do masking policies learned from a given task generalize beyond that task?
    \item \textbf{Q5.} How are these masking policies different from each other in terms of their masking decisions?
\end{itemize}

% (2) In which cases is intermediate pre-training helpful? Which masking policy tend to help which downstream tasks?
% (3) How are these masking policies different from each other in terms of their masking decisions?

To answer Q1 and Q2, we select eight downstream tasks from three categories (closed-book QA, knowledge-intensive language tasks, and abstractive summarization) and compare the downstream performance when different heuristic masking policies are adopted. Our results suggest that successful intermediate pre-training is dependent on availability of suitable in-domain corpus and sufficient pre-train scale. Moreover, heuristic-based approaches are effective when we have a precise understanding of the role that masked language modeling (MLM) plays in downstream task. For example, MLM serves as a sort of memorization step \cite{petroni-etal-2019-language}, whereby learning to unmask spans in context is analogous to memorizing facts about the span. However, in the absence of this understanding, it can be difficult to design a heuristic policy or make informed decisions. 

This lead us to Q3 and Q4, and explore whether learning masking policies is feasible. We design methods to learn a masking policy with supervised learning (\S\ref{sec:supervised-policy}) or meta-learning (\S\ref{sec:meta-learned-policy}), and compare downstream task performance using the same protocol in Q1 and Q2. Notably, we observe that masking policies learned with supervised learning and meta-learning outperforms the heuristic SSM policy for TriviaQA \cite{joshi-etal-2017-triviaqa}, and these policies learned from TriviaQA also help improve performance on Web Questions \cite{berant-etal-2013-semantic}. For Q5, we quantitatively compare the masks produced by different policies, including the distribution of part-of-speech tags among masked tokens, and their relation to token frequency in the corpus (\S\ref{sec:quant-analysis}). We find that the masking policies learned from TriviaQA tend to mask more proper nouns, and tend to mask less frequent words, when compared to SSM. 

We hope this work provide useful insights into how intermediate pre-training works and how masking policies influence downstream performance. Furthermore, we hope it would assist NLP researchers who aim to improve downstream task performance via intermediate pre-training, and invite future works on learned masking policies. 

% Our main findings include the following: .... \qinyuan{todo}
%Our analysis suggests that two important factors for successful intermediate pre-training are availability of in-domain corpus and computation resources. 
% Our main findings suggest that heuristic-based approaches can be effective when we have a precise understanding of the role that masked language modeling (MLM) plays in downstream task performance.
% For example, 
% % in closed-book QA, 
% prior work has shown that MLM pre-training serves as a sort of memorization step \cite{petroni-etal-2019-language}, whereby learning to unmask spans in context is analogous to memorizing facts about the span.
% This understanding helps \textit{inform} the way we design heuristics: since closed-book QA tends to focus on named entities and dates, SSM which masks these spans can be helpful.
% However, in the absence of this understanding, it can be difficult to make informed decisions.
% Why is MLM pre-training helpful for, say, summarization?
% Without knowing an explicit answer, it can be difficult to design the ``optimal" masking heuristic for summarization.
% In these cases, it may be beneficial to \textit{learn} a masking policy.
% We offer our suggestions for deciding the masking strategy in \S\ref{sec:discussion} and hope this work would assist NLP researchers who aim to improve downstream task performance via intermediate pre-training.


% \qinyuan{Limit the scope to knowledge intensive tasks or (more general) generation tasks?} \belinda{Should either figure out some way to argue summarization fits into knowledge-intensive tasks, or modify intro. (Either way should probably delete mentions of ``QA" in intro.) Also, not sure summarization works in same mechanism as closed-book qa (i.e. closed-book qa = memorizing knowledge from pretraining, summarization = memorizing ``knowledge" from current doc and compressing it--though maybe pretraining knowledge could still come in handy?) Should think harder about how we want to frame it...}

% Prior work has shown that large, neural language models (LMs) have a remarkable capability to learn knowledge from pre-training, which is stored implicitly within their parameters \cite{petroni-etal-2019-language}.
% This encoded knowledge allows LMs to perform a wide variety
% of knowledge-intensive tasks \textit{without} an external knowledge base, including %question-answering (QA), 
% knowledge base relation inference and fact checking~\cite{petroni-etal-2019-language, lee-etal-2020-language}.
% The implicit knowledge capacity can also be tested in the form of question answering, in the task termed as ``Closed-book QA" \cite{roberts2020much}. By directly fine-tuning the LM with (question, answer) pairs, closed-book methods perform competitively with retrieval-based methods on open-domain QA benchmarks.\footnote{Extremely large language models such as GPT-3~\cite{brown2020language} performed competitively on closed-book QA benchmarks without any fine-tuning (zero-shot).} 

% One integral component of the success of closed-book QA is \textit{salient span masking} (SSM, \citealt{guu2020realm}), an intermediate pre-training task that bridges general pre-training and task-specific fine-tuning by training the model to recover masked named entities or dates in the pre-training corpus (See Fig.~\ref{fig:intro} for illustration). 
% Notably, SSM brings 9\%+ EM improvement on TriviaQA \cite{joshi-etal-2017-triviaqa} when T5-11B is used. For comparison, scaling T5 model from 3B parameters to 11B only yielded 7\% improvements~---~indicating that a good choice of masking strategy could be even more influential than scaling the model size.

% % \input{figures_input/intro}

% This observation leads to our research question~---~How can we find a policy that generates masks more strategically? Such masking policy will pack more \textit{task-relevant} knowledge into the LM, and subsequently provide a better initialization for fine-tuning on closed-book QA tasks. In short, building upon 
% ``\textit{How much} knowledge can you pack into the parameters of a language model?'' 
% \cite{roberts2020much}, we seek to answer ``\textit{What} knowledge do you want to pack into the parameters of a language model?''


% To this end, we propose to learn a masking policy that models which spans in the pre-training corpus are likely to be queried, and thus, should be masked. Given a question $q$, an answer span~$a$, and the context passage $c$ that the answer is extracted from (usually given in the dataset), 
% % we make use of existing (context, question, answer) examples from downstream QA tasks and 
% we learn to extract answer span $a$ from context paragraph $c$, without prior knowledge of what the question $q$ is. 
% This masking policy is analogous to the ``gap selection'' model in question generation tasks \cite{becker-etal-2012-mind}. It is expected to capture a student's meta-knowledge when preparing for a closed-book exam: given a textbook, the student knows what contents are likely to be tested (presumably from previous experience of taking exams), and thus the student will try to focus on these contents.

% We use BART-base \cite{lewis-etal-2020-bart} as our backbone and extensively experiment with several masking policies learned from different sources of supervision. With a masking policy learned on TriviaQA, we achieve $24.71\%_{(\pm .21)}$ exact match on TriviaQA, surpassing $23.62\%_{(\pm .29)}$ using SSM and $22.93\%_{(\pm.14)}$ using random masking. The same trend holds when we deploy our best-performing policy to BART-large. We also observe that learned masking policies can positively transfer in some (but not all) cases: in these cases, a policy learned from one QA dataset can benefit other QA datasets.


==> sections/2_analysis_setup.tex <==
\section{Preliminary: Masked Language Modeling}

In this section, we revisit MLM objective with the notation that we will use throughout the paper. MLM is
a predominant pre-training objective for large-scale transformers in NLP
% self-supervised pre-training objective
\cite{devlin-etal-2019-bert}.
MLM and its variants can be characterized with two key components:
a \textbf{masking policy} $g(.;\phi)$, parameterized by $\phi$, which decides the collection of tokens to be masked, and 
a \textbf{language model} $f(.;\theta)$, parameterized by $\theta$.

Formally, given a sequence of tokens $\mathbf{x}=[x_1, x_2, ..., x_m]$, %in the pre-training corpus, 
$g(\mathbf{x};\phi)$ generates a sequence of binary decisions $\mathbf{d}=[d_1, d_2, ..., d_m]$, where $d_i=1$ indicates the token $x_i$ will be masked.
% The tokens $\mathbf{x}$ and the decisions $\mathbf{d}$ will go through a post-processing step, where a source sequence $\mathbf{x}^{(\text{src})}$ and a target sequence $\mathbf{x}^{(\text{tar})}$ are determined.
The source sequence for pre-training, $\mathbf{x}^{(\text{src})}$, is formulated by replacing the selected tokens with a special \texttt{<mask>} token, i.e., $\mathbf{x}^{(\text{src})}=[x^{(\text{src})}_1, x^{(\text{src})}_2, ..., x^{(\text{src})}_m]$, where $x^{(\text{src})}_i=x_i$ if $d_i=0$ and $x^{(\text{src})}_i=\texttt{<mask>}$ if $d_i=1$. We denote this operation as $\mathbf{x}^{(\text{src})} = \mathbf{x} \oplus \mathbf{d}$. The target sequence $\mathbf{x}^{(\text{tar})}$ can be either the full original sequence $\mathbf{x}$ (BART, \citealt{lewis-etal-2020-bart}), or the sequence of masked tokens (T5, \citealt{raffel2019exploring}).
% In salient-span masking (SSM), $g$ is .... In BART pretraining, $g$ is.... \bzl{can we add a sentence about how SSM works (using our notation) here?}

\section{Analysis Setup}
\label{sec:analysis-setup}

% Our goal is to analyze the influence brought by different masking policies during intermediate pre-training. 
% The only variable is the masking policy, while other aspects are controlled. The influence is measured by the performance on downstream tasks. 
In this section we introduce the analysis pipeline (\S\ref{sec:analysis-pipeline}) and downstream datasets we use (\S\ref{sec:downstream-tasks}). 
We defer the details of learned masking policies to \S\ref{sec:compared-policies}.


\subsection{Experiment Procedure} 
\label{sec:analysis-pipeline}
Our goal is to analyze the influence in downstream task performance brought by different masking policies $g(.;\phi)$ during intermediate pre-training. Towards this goal, we ensure that the only variable is the masking policy, while all other aspects are controlled, so that the downstream performance reveal the influence we aim to study.
We first initialize with a BART-base \cite{lewis-etal-2020-bart} model pre-trained on open-domain data.
Then for each masking policy, we conduct experiments following a two-stage pipeline: 

\paragraph{Stage 1. Intermediate Pre-training.} We perform intermediate pre-training with a given masking policy $g(.;\phi)$.
Unless stated otherwise, all intermediate pre-training is done with input sequence length of 128, batch size of 2048, learning rate of $0.0001$, up to a total number of $100,000$ updates, using Wikipedia snapshot from December 20, 2018\footnote{The snapshot is available at \url{https://archive.org/download/enwiki-20181220}. Wikipedia is licensed under \href{https://creativecommons.org/licenses/by-sa/3.0/}{CC BY-SA 3.0}.}. The learning rate linearly increase to $0.0001$ in the first 6\% of the updates, and linearly decreases to $0$ in the remaining steps. 
% See Appendix \ref{app:hps-intermediate} for details.

\paragraph{Stage 2. Task-specific Fine-tuning.} We fine-tune each resulting checkpoint from Stage 1 on related downstream tasks, and evaluate their performance. We follow the same routine of hyperparameter search for each checkpoint. We then run the fine-tuning experiments with the best hyperparameter setting and three different random seeds. See Appendix \ref{app:hps-downstream} for details. 

\subsection{Downstream Tasks and Datasets} 
\label{sec:downstream-tasks}
We focus our study on eight tasks across three categories. We introduce their details and explain the rationale behind our selection in the following.
% \bzl{what if we added a bit of intuition here on what we think the learned masking will do in each case (i.e. in case of cloesd-book qa, it's learning what "knowledge" to pack). idk if it's helpful here or do all analysis post-hoc}

\paragraph{Closed-book QA.} Closed-book QA is a task that requires language models to directly answer questions without access to external knowledge \cite{roberts-etal-2020-much}. This paradigm assumes that the model memorizes large amounts of knowledge from its pre-training data, which gets ``packed" into its parameters, and can subsequently be ``retrieved" to answer questions.
Notably, \citet{roberts-etal-2020-much} reported 9\%+ improvement in exact match on TriviaQA when intermediate pre-training with salient span masking (\textit{i.e.}, masking and recovering named entities or dates) is performed on a T5-11B model. This observation inspired our work. Our study considers three datasets for closed-book QA: Natural Questions (\textbf{NQ}, \citealt{kwiatkowski-etal-2019-natural}), WebQuestions (\textbf{WQ}) and \mbox{TriviaQA} (\textbf{TQA}).


\paragraph{Knowledge-Intensive Tasks (KILT).} 
% In order to explore whether salient span masking generalizes to other tasks that requires implicit knowledge stored in the LM, we select three tasks from the KILT benchmark \cite{petroni2020kilt} and conduct experiments in implicit knowledge setting (\textit{i.e.}, without retrieving external knowledge). 
Extending from closed-book QA, we select three tasks from the KILT benchmark \cite{petroni2020kilt} that also aims to test a model's implicit knowledge capacity, while having different task formats and goals.
Aidayago2 (\textbf{AY2}, \citealt{hoffart-etal-2011-robust}) is an entity linking task that requires the model to assign a Wikipedia page to an entity mention in the text. The output is the unique name of the Wikipedia page in text format. 
Zero-shot relation extraction (\textbf{ZSRE}, \citealt{levy-etal-2017-zero}) is a slot filling task that aims to predict the object when given the subject and the relation. The relations in the train/dev/test splits are non-overlapping.
Wizard of Wikipedia (\textbf{WoW}, \citealt{Dinan2019WizardOW}) is a dataset of dialogue histories relevant to knowledge in Wikipedia. The model is required to act like a chatbot and generate the response given previous dialogue history.

\paragraph{Abstractive Summarization.} Inspired by recent work that pre-trains LMs with gap sentence generation (masking and recovering whole sentences, \citealt{Zhang2019PEGASUSPW}), we explore heuristic and learned policies during intermediate pre-training for abstractive summarization. We use the CNN/Daily Mail (\textbf{CNN/DM}, \citealt{NIPS2015_afdec700}) and Extreme Summarization (\textbf{XSum}, \citealt{narayan-etal-2018-dont}) datasets. For CNN/DM, the summaries are similar to source sequences, while the summaries in XSum are more concise and abstractive.

\vspace{0.5cm}
All tasks above can be treated as sequence-to-sequence tasks, where each example is a source-target pair $(\mathbf{s}, \mathbf{t})$. For closed-book QA and KILT tasks, each $(\mathbf{s}, \mathbf{t})$ is accompanied with a context paragraph $\mathbf{c}$ that provides provenance for the answer $\mathbf{t}$. For summarization tasks, we approximate this by treating the source sequence $\mathbf{s}$ as context paragraph $\mathbf{c}$. %as an approximation.
%In later sections, we introduce how we learn masking policies from these $(\mathbf{c}, \mathbf{s}, \mathbf{t})$ examples.

% \subsection{Compared Masking Policies.} We include three categories of masking policies in our study: (1) Heuristics, including the denoising objective used to train BART \cite{lewis-etal-2020-bart}, random masking, and salient span masking. (2) Supervised policy (Sec. \ref{sec:supervised-policy}). (3) Meta-learned policy (Sec. \ref{sec:meta-learned-policy}). We defer the technical details of learned policies in later sections.

% \paragraph{Problem Definition.} 
% Our goal is to learn a masking policy $g(.;\phi)$ that helps ``pack" task-relevant knowledge into LM parameters (Stage~1 in Fig.~\ref{fig:concept}). To effectively learn the masking policy, we assume access to (context, question, answer) examples for at least one QA dataset\footnote{The context can be annotated by humans (Natural Questions) or obtained from distant supervision (TriviaQA). The latter requires simple retrieval methods such as BM25.}, which we refer to as \textit{anchor task(s)}. 
% To evaluate a learned policy, we deploy it in intermediate pre-training (Stage 2), on a preset corpus (\textit{i.e.}, Wikipedia), then fine-tune on downstream closed-book QA tasks (Stage 3). 

% \input{figures_input/stages}



==> sections/3_method.tex <==
\section{Compared Masking Policies}
% In this section, we introduce the three categories of masking policies that are compared in this work
We experiment with three categories of masking policies:  %. Namely, we introduce 
heuristic policies, where $g$ is a fixed heuristic function (\S\ref{sec:heuristic-policies}); supervised policies, where $g$ is a model whose weights are learned from \textit{direct supervision} on downstream tasks (\S\ref{sec:supervised-policy}); and meta-learned policies, where $g$ is a model whose weights are learned through \textit{meta-learning} on downstream tasks (\S\ref{sec:meta-learned-policy}).

\label{sec:compared-policies}
\subsection{Heuristic Policy}
\label{sec:heuristic-policies}
% We take the publicly released BART-base model as the starting point, and include the following heuristic masking policies as baselines:
We experiment with the following heuristic masking policies:
(1) Intermediate pre-training with BART's original objective (+Orig);
(2) Intermediate pre-training by masking and recovering 15\% randomly selected tokens (+Rand)\footnote{15\% is borrowed from BERT and T5. ``+Orig'' and ``+Rand'' are different in that $\mathbf{x}^{\text{(tar)}}=\mathbf{x}$ for ``+Orig'', while $\mathbf{x}^{\text{(tar)}}$ contains the masked 15\% tokens for ``+Rand''.}; 
(3) Intermediate pre-training with salient span masking \cite{roberts-etal-2020-much, guu2020realm} (+SSM);

For summarization tasks, we include two additional heuristics:
(4) Intermediate pre-training by randomly masking 30\% sentences (+MaskRandomSent);
(5) Intermediate pre-training by masking the first 30\%\footnote{Borrowed from BART's original masking probability.} sentences (+MaskFirstSent).

\subsection{Supervised Policy}
\label{sec:supervised-policy}

When students prepare for closed-book exams, they are likely to review and memorize what they perceive as most important in the text book. Such perception is learned from their prior experience of taking closed-book exams. Following this intuition, \citet{Ye2020StudyingSL} proposed to learn a masking policy for closed-book QA tasks to help the model focus on \textit{likely answers} during intermediate pre-training. The masking policy is trained with (answer, context) examples, and the policy is an extractive model that extracts the answer span from the context. In the following, we briefly recap the method and extend to more task formats (e.g., knowledge-intensive tasks and summarization) with our notations.

% \qinyuan{need to re-write this so we can cite ``studying strategically'' paper.}
% When preparing for a closed-book exam, students focus on content that is likely to be tested, selecting this content based on prior exam-taking experience. Inspired by this, we propose to mask \textit{likely answers} from an evidence document, such that during the pre-training phase, the language model will focus on ``memorizing", or learning to unmask, spans that resemble answers.
% We identify these spans by directly training a masking model on $(\mathbf{c}, \mathbf{t})$ examples\footnote{Supervised policy requires that $\mathbf{t}$ appears as is in $\mathbf{c}$.}, which we will detail below.

\paragraph{Overview.} Following SSM, we mask and reconstruct exactly one span, so $g(\mathbf{x};\phi)$ can take an equivalent form of predicting the start and end positions of a span. Given a set of triplets $(\mathbf{c}, \mathbf{s}, \mathbf{t})$, we learn $g(\mathbf{x};\phi)$ from $(\mathbf{c}, \mathbf{t})$ pairs only, training our policy to extract the \textit{target} from within the \textit{context}. Following \cite{Ye2020StudyingSL}, we use a lightweight architecture (2-layer Bi-LSTM model with one linear layer) to avoid computation bottleneck.

%At a high level, we want to learn to mask \textit{likely answers/targets} from an evidence document, such that during the pre-training phase, the language model will focus on ``memorizing", or learning to unmask, spans that resemble answers/targets.

% Since the policy will be deployed to make masking decisions on a massive pre-training corpus, we opt to use light-weight architectures instead of larger transformer models. We encode the context sequence with a 2-layer Bi-LSTM model, then use a linear layer to predict the start and end positions of a potential answer span.
% \qinyuan{I'm confused... If we're going to cite ``studying strategically'' and submit a separate arxiv paper, what do we put here?}
\paragraph{Model.} %More specifically, g
Given context paragraph tokens $\mathbf{x}=[x_1, x_2, ..., x_m]$, we first use an embedding matrix $\mathbf{E}$ to embed each token: $[\mathbf{e}_1, \mathbf{e}_2, ..., \mathbf{e}_n]$. Then, we use a 2-layer bidirectional LSTM model to compute the hidden representation at each position. 
\vspace{-0.1cm}
\begin{equation}
    [\mathbf{h}_1, \mathbf{h}_2, ..., \mathbf{h}_n] = \textrm{Bi-LSTM}([\mathbf{e}_1, \mathbf{e}_2, ..., \mathbf{e}_n])
\end{equation}

Finally, we use two learned vectors $(\mathbf{w}_{st}, b_{st})$ and $(\mathbf{w}_{ed}, b_{ed})$ to compute the logits for each position being the start or end position of the potential answer/target span. For example, the logit of position $j$ being a start/end position is computed as follows.
\vspace{-0.1cm}
\begin{equation}
\begin{aligned}
    y_{j, st} = \mathbf{w}_{st} \mathbf{h}_j + b_{st},
    \ \  y_{j, ed} = \mathbf{w}_{ed} \mathbf{h}_j + b_{ed}.
\end{aligned}
\end{equation}

\paragraph{Policy Inference.} When deploying the policy to intermediate pre-training, we select the potential answer spans by ranking the sum of start and end logits of each potential spans, in accordance to the inference step in machine reading comprehension models. That is, we rank the spans $(i,j)$ according to $y_{i, st}+y_{j, ed}$. We consider two variants when deploying the policy: (a) masking the top 1 span or (b) sampling 1 span from the top 5 spans.

\paragraph{Extending to Other Tasks.} Supervised policy is designed for closed-book QA, and one limitation of this method is that the target span $\mathbf{t}$ must appear as is in the context paragraph $\mathbf{c}$. Within the three selected knowledge intensive tasks, ZSRE satisfy this constraint. For summarization tasks, we design a workaround by leveraging the extractive summaries of CNN/DM dataset produced by MatchSum \cite{zhong-etal-2020-extractive}. In this case, $\mathbf{c}$ is the original document to be summarized, and $\mathbf{t}$ is one full sentence that appear in the extractive summary. To sum up, we apply supervised policy to TQA, NQ, ZSRE and CNN/DM.

\subsection{Meta-learned Policy}
% \input{algorithm/algo-metalearn}
\label{sec:meta-learned-policy}

% \xiang{before going into tech details, say sth about why we want to look at this policy --- any unique characters vs. other policies in comparison?}
Conceptually, what the learned masking policy captures is closely related to the concept of ``learning to learn'' \cite{schmidhuber1987evolutionary, thrun2012learning}. At a high level, the masking policy should provide the model with the desired initialization for the downstream task, such that the model can better learn the downstream task in only a few fine-tuning updates. Therefore, we construct a meta-learning approach, which we describe below. %We formally describe this method below. 
% Additional details can be found in Appendix~\ref{}.%in the following.

\paragraph{Overview.}
We formulate each $(\mathbf{c},\mathbf{s},\mathbf{t})$ example as a small task. For each task, the goal is to improve the performance of generating target sequence $\mathbf{t}$ given input $\mathbf{s}$, immediately after learning from the context $\mathbf{c}$. This is similar to taking quizzes, where a student first learns from a passage $\mathbf{c}$ and then is immediately tested on it by trying to answer $\mathbf{t}$ given $\mathbf{s}$. Studying from $\mathbf{c}$ strategically with an optimal masking policy will result in better performance on this quiz (\textit{i.e.}, smaller loss in generating $\mathbf{t}$).

Following work in gradient-based meta-learning \cite{pmlr-v70-finn17a, grefenstette2019generalized}, we set up an \textit{inner} and \textit{outer} loop. We briefly sketch the procedure in Fig. \ref{fig:meta-learn}.
In the inner loop, we focus on the current $(\mathbf{c},\mathbf{s},\mathbf{t})$ examples by applying the current masking policy $g(.;\phi)$ and performing pre-train/fine-tune updates to $f(.;\theta)$. In the outer loop, we update the policy $g(.;\phi)$ with the signal at the end of inner loop training. We denote $\phi^{(p)}$ as the masking policy parameters after $p$ outer loop optimization steps, and $\theta^{(p,q)}$ as the LM parameters after $p$ outer loop optimization steps and $q$ inner loop optimization steps.

\input{figures/metalearn}
\paragraph{Inner Loop.} In one inner-loop curriculum, we first take the context as a pre-training sentence, \textit{i.e.}, $\mathbf{x}=\mathbf{c}$, and use the current masking policy $g(.;\phi^{(p)})$ to determine the masks $\mathbf{d}$ and the implied perturbed input $\mathbf{x}^{(\text{src})}$, \textit{i.e.}, $\mathbf{d} = g(\mathbf{x};\phi^{(p)})$, $\mathbf{x}^{(\text{src})} = \mathbf{x} \oplus \mathbf{d}$.
% \begin{align}\label{eq:meta-start}
%     \mathbf{d} = g(\mathbf{x};\phi^{(p)}), \ \ 
%     \mathbf{x}^{(\text{src})} = \mathbf{x} \oplus \mathbf{d}.
% \end{align}

We pre-train $\theta^{(p,0)}$ for one step to recover $\mathbf{x}$ from $\mathbf{x}^{(\text{src})}$:
\begin{equation}\label{eq:meta-start}
    \theta^{(p,1)} = \theta^{(p,0)} - \alpha_0 \nabla_{\theta^{(p,0)}}\mathcal{L}(f(\mathbf{x}^{(\text{src})};\theta^{(p,0)}), \mathbf{x}),
\end{equation}
where $\alpha_0$ is the learning rate, and $\mathcal{L(.,.)}$ is the cross entropy loss for recovering $\mathbf{x}$ using disturbed input $\mathbf{x}^{(\text{src})}$ and model parameters $\theta^{(p,0)}$.

Next, we take $\theta^{(p,1)}$ as initialization and fine-tune it for one step on the downstream objective of predicting $\mathbf{t}$ given $\mathbf{s}$: 
\begin{equation}
    \theta^{(p,2)} = \theta^{(p,1)} - \alpha_1 \nabla_{\theta^{(p,1)}}\mathcal{L}(f(\mathbf{s};\theta^{(p,1)}), \mathbf{t}).
\end{equation}

\paragraph{Outer Loop.} In outer loop, we update the masking policy $g(.;\phi^{(p)})$.
We aim to answer query $\mathbf{s}$ correctly after the inner-loop curriculum. We define the meta-loss $\mathcal{L}'$ as the decrease in losses after the one fine-tuning update, \textit{i.e.},
\begin{equation}\label{eq:meta-end}
    \mathcal{L}' = \mathcal{L}(f(\mathbf{s};\theta^{(p,2)}), \mathbf{t})-\mathcal{L}(f(\mathbf{s};\theta^{(p,1)}), \mathbf{t}).
\end{equation}
$\mathcal{L}'$ characterizes how fast the model has adapted itself to answer ($\mathbf{s}$, $\mathbf{t}$) within one step of optimization.
Since all computations in Eq. (\ref{eq:meta-start}-\ref{eq:meta-end}) are continuous\footnote{We use Gumbel Softmax \cite{Jang2017CategoricalRW} to discretize the output of $g(.;\phi^{(p)})$ and formulate masking decision $\mathbf{d}$, and we use embedding mixture for $\mathbf{x}^{(\text{src})} = \mathbf{x} \oplus \mathbf{d}$}, we can optimize $\phi$ by directly taking gradients from $\mathcal{L}'$, \textit{i.e.},
\begin{equation}
    \phi^{(p+1)} = \phi^{(p)} - \alpha_2 \nabla_{\phi^{(p)}}\mathcal{L}'.
    \label{eq:outer_raw}
\end{equation}
% \paragraph{Other Details.} 
% Due to space limit, we leave additional details such as design choices of $g(.;\phi^{(p)})$, controlling masking budget, and post-processing in Appendix \ref{app:meta}.

\paragraph{Controlling Masking Budget.} Higher order optimization is known to be unstable \cite{antoniou2018how}. In early stages of the study, we found the policy to be flipping between masking none or all of the tokens. To stabilize, we add a softened L2 loss to control the portion of mask/not-mask decisions output by $g(.;\phi)$. Denoting $l(\mathbf{x})$ as the input sequence length, $l(\mathbf{d})$ as the number of mask decisions; we define a budget $\gamma$ and a tolerance factor $\epsilon$, and compute the regularization term $\mathcal{L}_{reg}$,

\begin{equation}
\small
\mathcal{L}_{reg}(\mathbf{x}, \mathbf{d})=\left\{
\begin{aligned}
 & 0, \quad |\gamma l(\mathbf{x}) - l(\mathbf{d})| \leq \epsilon l(\mathbf{x}) \\
%  ((\gamma-\epsilon)l(\mathbf{x}') \leq l(\mathbf{x}'') \leq (\gamma+\epsilon)l(\mathbf{x}')\\
 & (\gamma l(\mathbf{x}) - l(\mathbf{d}))^2, \quad \text{otherwise}
\end{aligned}
\right.
\label{eq:budget}
\end{equation}

For example, when $\gamma=15\%$, $\epsilon=5\%$ and the input sequence $\mathbf{x}$ contains 100 tokens, the policy will not be penalized if it's masking $15\pm5$ of all tokens in the sequence. We modify the optimization step in Eq. (\ref{eq:outer_raw}) as follows, where $\beta$ is a co-efficient balancing the regularization intensity.
\begin{equation}
    \phi^{(p+1)} = \phi^{(p)} - \alpha_2 \nabla_{\phi^{(p)}}(\mathcal{L}' + \beta \mathcal{L}_{reg}(\mathbf{x}, \mathbf{d}))\\
\end{equation}

\paragraph{Post-processing.} When we deploy a learned policy to pre-training, we are no longer constrained by differentiability. Based on useful techniques in previous work, we apply post-processing to predicted masking decisions $\mathbf{d}$. (1) Whole-word masking and text infilling \cite{liu2019roberta, lewis-etal-2020-bart}: whenever one subword $x_i$ within a whole word is masked ($d_i=1$), we expand the mask and always mask the whole word. When consecutive tokens are masked, we replace the sequence of \texttt{<mask>} in the input sequence with exactly one \texttt{<mask>} token. (2) Additional budget control: Even with our budget regularization loss (Eq. \ref{eq:budget}), we find some input sequences get too many masks ($>50\%$). This creates extremely challenging pre-train examples that may prevent the model from learning useful information. For these sentences we randomly ``unmask'' tokens to keep the portion of masks below $30\%$.

==> sections/4_experiment.tex <==
\section{Results and Discussion}

\label{sec:exp-results}
Following our analysis setup, we list the results for closed-book QA tasks in Table \ref{tab:cbqa}, knowledge-intensive language tasks in Table \ref{tab:kilt} and summarization tasks in Table \ref{tab:summarization-simplified}. In the following, we revisit and try to answer the question we raised in the introduction. 
% We hope our analysis offer suggestions to NLP researchers and practitioners who wish to improve downstream performance via intermediate pre-training.

\input{tables/closed-book}
\input{tables/kilt}
\input{tables/summarization_simplified}

\noindent \textbf{Q1. Is intermediate pre-training helpful?} Prior work has shown that intermediate pre-training on \textit{encoder} models (i.e., RoBERTa, \citealt{liu2019roberta}) with in-domain corpora helps to improve downstream \textit{classification} tasks performance \cite{gururangan-etal-2020-dont}. Our experiments help to examine whether similar conclusion holds for text-to-text transformers and other NLP tasks. In our experiments, we found intermediate pre-training with Wikipedia and BART's original objective (+Orig) help improve performance of two closed-book QA tasks (TQA and WQ) and one entity linking task (AY2). However, for summarization tasks, intermediate pre-training mostly hurts performance. We conjecture the reason to be (1) using a smaller sequence length (128) in our experiments as compared to general pre-training of BART (512); or (2) using Wikipedia as pre-train corpus, while summarization data are mostly news articles. To conclude, pre-training on \textit{appropriate in-domain corpora} with a \textit{sufficient pre-training scale} (batch size, sequence length) are prerequisites for intermediate pre-training to work. For Q1, we focus on intermediate pre-training with the original objective, though the conclusion varies when heuristic and learned masking policies are introduced, which we discuss in Q2 and Q3.
% For closed-book QA and knowledge-intensive tasks, continue pre-training with Wikipedia, with the original objective, is bringing improvements 
% Our experiments on summarization suggest pre-training on an \textit{out-of-domain corpus} with promising heuristics or masking policies, or with \textit{smaller pre-training scale} (batch size, sequence length), would hurt final performance. Lack of in-domain corpus or sufficient computation resources may lead to in-successful intermediate pre-training.

\noindent \textbf{Q2. Among heuristic policies, which one should be used during intermediate pre-training?} From the results in Table \ref{tab:cbqa}, we first confirm that salient span masking (SSM) is indeed very beneficial for closed-book QA \cite{roberts2020much}. In addition, SSM helps improve performance for two entity-centric knowledge intensive tasks (AY2 and ZSRE, see Table \ref{tab:kilt}). Though Wikipedia is not the ideal pre-train corpus for summarization tasks, in Table \ref{tab:summarization-simplified} the results suggest masking random sentence is the best one among all heuristic masking policies. We conclude that heuristic masking policies that resemble the downstream tasks tend to improve downstream performance, as SSM resembles closed-book QA and gap sentence generation resembles summarization to some extent. When it's hard to design a heuristic that resemble downstream task, using random masking on in-domain corpus may be helpful. In this case, we recommend to decide whether to generate full sequence (+Orig) or only masked tokens (+Rand) based on the task output length. If the downstream tasks requires generating full sentences (\textit{e.g.}, dialogue, summarization), generating full sequence is more helpful. This is supported by the observation that +Orig is better than +Rand for WoW, CNN/DM and XSum. On the other hand, if the target sequences in the downstream dataset are shorter, generating masked tokens is more helpful, as shown by experiments on NQ, AY2 and ZSRE.

\noindent \textbf{Q3. Can learned policies be better than heuristics?} Our short answer is: it depends on the downstream tasks, and there is still much room to explore for this question. From our experiments we see that learned policies are most successful on TriviaQA, with both the supervised policy and the meta-learned policy outperforming SSM. We attribute its success to the following reasons: (1) (context, source, target) examples are abundant, so the masking policy has sufficient supervision. TriviaQA dataset is accompanied with large-scale context paragraphs created with distant supervision, so the scale of $(\mathbf{c}, \mathbf{s}, \mathbf{t})$ examples is larger than other datasets. (2) The heuristic masking policy does not ``perfectly'' resemble the downstream task, and still has room to improve. SSM masks one random named entity in the context. However, the answer to trivia questions are not necessarily named entities, and one named entity may be more important than than another. Therefore the learned policy can better capture the characteristics of TriviaQA than SSM. When these conditions are satisfied, learned masking policies are worth trying. Apart from TriviaQA, meta-learned policies outperforms +Orig on NQ, ZSRE and WoW, demonstrating the effectiveness of the method. This also opens up a way for tasks whose heuristic masking policy is not intuitive (e.g., dialogue response generation tasks such as WoW). The two methods for learning masking policies are just our initial attempt towards the idea of ``learning to mask'', and we hope future work investigate the issues such as over-fitting of the masking policy and instability in meta-learning, and design novel methods to learn a masking policy.

\noindent \textbf{Q4. Are masking policies transferable?} We observe several cases where a policy learned from one dataset positively transfer to another downstream tasks. That includes Supervised-TQA(Top5) bringing improvement to WQ, +Supervised-NQ(Top5) bringing improvement to TQA, and +Supervised-ZSRE(Top5) bringing improvement to AY2, compared to random masking baselines. This is reasonable since all these tasks are entity-centric and are similar in nature. For tasks with significantly different formats and goals, e.g., ZSRE and WoW, policies learned on one does not benefit another. Here we only exhibit the evidence supporting that learned masking policies can be transferable, and we leave the question of ``when and why does it work'' as future work.



==> sections/5_analysis.tex <==
\section{Analysis of Masking Policies}
\label{sec:quant-analysis}
\input{figures/pos-tags}
% \textbf{How are these masking policies different from each other?}
To answer the last question we raised, \textbf{``How are these masking policies different from each other in terms of their masking decisions?''},  we analyze the correlation between masking decisions and part-of-speech tags and token frequency. Specifically, we take 1\% of the pre-train corpus and compare the decisions made by each masking policy to facilitate our analysis.

\subsection{Relation to Part-of-speech Tags}
In Fig. \ref{fig:pos-tag}, we plot the stacked bar chart of part-of-speech tags to visualize their distribution. Each bar represent the portion of masks having the part-of-speech tag, amongst all masks produced by this policy. Notably, most \textit{supervised} policies learns to focus more on proper nouns, and less on common nouns. This is consistent with the goal of the downstream tasks such as NQ and TQA. Comparing Supervised-TQA and SSM, we see that Supervised-TQA focuses less on nouns, numbers and adjectives, and it focuses even more on proper nouns. This suggests that Supervised-TQA better characterizes the property of TQA, and thus outperforms SSM by learning to mask task-specific information.

Due to the differences in learning procedures, the \textit{meta-learned} policies has distributions different from supervised policies. Still, meta-learned policies for NQ and TQA masks more nouns, proper nouns, and fewer adpositions. For WoW, whose heuristic masking policy is less clear, the meta-learned policy tend to mask more nouns and fewer verbs, compared to the random masking baseline.

\subsection{Relation to Token Frequency}
In Fig. \ref{fig:freq}, we plot the relation between mask frequency and token frequency for masking policies learned from TQA, along with random masking and SSM for reference. Mask frequency is computed as the number of occurrences that a token was masked divided by the number of all masked tokens. For random masking, the datapoints approximate a Zipfian distribution, with some noise due to random sampling of words \cite{zipf1999psycho}. Secondly, for SSM, most datapoints fall on a curve that is above the random masking line, and another portion of tokens are less likely to be masked, formulating line segments in the bottom area. The SSM policy shows a wider distribution around the line $1 / x$ than the random masking policy, indicating that it has a strong preference for specific tokens, and a weaker preference for Zipfian behavior.
% This suggests a portion of tokens are seldom masked according to SSM. 
For the Supervised-TQA (Fig. \ref{fig:freq}(a)) and Meta-TQA (Fig. \ref{fig:freq}(b)) policies, we observe an even stronger preference for specific tokens. Both policies show a stronger preference for less frequent tokens than the random masking policy.

% we observe that a line segment between frequency rank of $200$ and $2000$ overlaps with the random masking baseline, but is more thick and scattered. 
% We then observe a dense yellow area above random masking baseline between frequency rank $10000$ and $40000$. This suggests Supervised-TQA policy is more likely to mask less frequent tokens. We observe a similar trend in Fig. \ref{fig:freq}(b) for the meta-learned policy for TQA. This suggests that though supervised policy and meta-learned policy are different in methodology, the meta-knowledge learned by both methods may be similar. 

% For Supervised-CNN/DM (Fig. \ref{fig:freq}(b)), the plot mostly overlap with random baseline, though having more scatters around the major line. 
% For Meta-learned-WoW, the plot is mostly above the random masking policy, while being below the Meta-learned-TQA policy.

% \subsection{Visualizing in 2D Space}
\input{figures/frequency}
% % \todo{the frequency figure will slower the latex compilation. deleting for now but will add back.}
% \input{figures/2d_visualization}
% Fig. \ref{fig:2d} visualizes the similarity between different masking policies. We take one minus the average cosine similarities of masking decisions made for pre-train examples as the distance between two policies, and use multi-dimensional scaling algorithm to project to 2D space. We observe that policies learned from TQA and ZSRE are close to SSM in both figures, which is in line with the observation that a majority of the targets in these two datasets are named entities and dates. We also see that policies learned from closed-book QA and knowledge-intensive tasks tend to be close to each other, since both categories examine a model's capacity of implicit knowledge.

==> sections/7_conclusion.tex <==
\section{Conclusion}
From extensive experiments with heuristic and learned masking policies across three types of tasks, we have identified several successful cases of intermediate pre-training, offered in-depth analysis and insights for the masking policies we used, and summarized several suggestions for researchers who aim to improve model performance via intermediate pre-training. We believe that future work can expand on our methods, and search the space of pre-training objectives beyond masked language modeling. Furthermore, we hope our work encourages researchers to consider the type of downstream applications they wish to deploy their LMs in, before investing resources into large-scale pre-training.

% pretraining methodologies
% carefully thinking 
% In particular
% In this paper we propose a simple and intuitive method to encode task-relevant knowledge into language models during intermediate pre-training. Our method resembles how students would prepare for a closed-book exam: reading the books in advance (pre-training on Wikipedia), figuring out what contents would likely appear in the test, and focusing on that content (by masking task-relevant spans). We showed the learned policy is particularly effective on TriviaQA; meanwhile the trend is less clear on other datasets, for which we discussed the reasons behind. We also observe some cases where a policy learned on one QA dataset can positively transfer to help improve performance of another, suggesting that the meta-knowledge captured by the learned policy can be transferable. 

% There are several potential directions for future work. 
% Firstly, what the masking policy captures is closely related to the concept of ``learning to learn'', and thus future work may exploit meta-learning methods to learn the masking policy. 
% Secondly, given recent advances in unsupervised QA \cite{lewis-etal-2019-unsupervised, shwartz-etal-2020-unsupervised}, it would be interesting to enable self-training by forming a closed-loop system that learns to memorize knowledge, ask questions, and provide answers.
% The success of the proposed approach motivates future work

\paragraph{Acknowledgments} 
We would like to thank Sebastian Riedel, Edward Grefenstette, Patrick Lewis, Xian Li and INK Lab members for the insightful discussions. Qinyuan Ye's research is supported in part by the Office of the Director of National Intelligence (ODNI), Intelligence Advanced Research Projects Activity (IARPA), via Contract No. 2019-19051600007.

==> sections/x_related_work.tex <==
\section{Related Work}

\paragraph{Implicit Knowledge in Pre-trained Language Models.} 
\citet{petroni-etal-2019-language} discovered that pre-trained language models can implicitly store relational knowledge in their parameters, and such knowledge can be accessed with cloze-style queries. \citet{roberts2020much} introduced the task of closed-book QA, which breaks the convention of retriever-reader strategy for open-domain QA, and requires the model to directly generate answers with its implicit knowledge. Closed-book QA performance is boosted significantly when salient span masking \cite{guu2020realm} is used. \citet{guu2020realm} maintained that SSM helps the model to ``focus on problems that require world knowledge''.

\paragraph{Self-supervised Pre-training.} 
Pre-trained language models has shown its capability on a wide variety of NLP tasks. Current self-supervised objectives are mostly \textit{heuristic}, including masked language modeling \cite{devlin-etal-2019-bert}, span boundary representation learning \cite{joshi-etal-2020-spanbert}, corrupted sentence reconstruction \cite{lewis-etal-2020-bart}, gap sentence generation \cite{Zhang2019PEGASUSPW}, etc. \citet{raffel2019exploring} systematically studied the self-supervised objectives used in previous literature. Related to our goal of exploring pre-training objectives, ELECTRA \cite{clark2020electra} propose a replaced token prediction task which improves pre-training efficiency. \citet{chen2020variance} propose to reduce the variance of gradients in SGD and expedite model pre-training. \citet{Levine2020pmimasking} propose to mask n-grams according to Pointwise Mutual Information (PMI). These works typically consider the efficiency of an objective when pre-training \textit{from scratch} and without preconceived focus on a given problem; while we focus on encoding knowledge or adapting the model during intermediate pre-training with a given task in mind.

\paragraph{Domain/Task-specific Pre-training.}
\citet{gururangan-etal-2020-dont} experiment on four domains (bio-medical, computer science, news, reviews) and eight different datasets, where they discover that pre-training with in-domain corpus leads to better downstream performance. \citet{vu-etal-2020-exploring, pruksachatkun-etal-2020-intermediate} studies intermediate-task transfer between NLP tasks. \citet{kang-etal-2020-neural} propose to learn a mask generator during task-specific pre-training via reinforcement learning. Closely related to us, \citet{gu-etal-2020-train} propose task-guided pre-training by first learning to predict importance score for each token and then launch task-specific pre-training by masking important tokens. 


==> tables/analysis.tex <==
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
                        & \%Mask & \%NE & \%NC \\
\midrule
BART-Base               & - & - & - \\
\midrule
Supervised-TQA & 2.73 & 72.59 & 85.11 \\
Supervised-NQ & 3.81 & 62.69 & 74.67 \\
Supervised-All & 3.19 & 71.67 & 82.95 \\
Supervised-ZSRE & 3.32 & 64.65 & 78.64 \\
Supervised-CNN/DM & 3.36 & 25.50 & 56.17 \\
\midrule
Meta-learned-TQA & 22.98 & 44.10 & 73.01 \\
Meta-learned-NQ & 26.43 & 35.05 & 72.96 \\
Meta-learned-ZSRE & 25.90 & 38.32 & 73.09 \\
Meta-learned-WoW & 26.34 & 23.56 & 49.60 \\
Meta-learned-CNN/DM & 26.19 & 37.88 & 69.49 \\
Meta-learned-XSum & 25.15 & 37.07 & 68.68 \\
\bottomrule
\end{tabular}
}
\caption{Statistics of the masks produced by the learned policies.}\label{tab:analysis}
\end{table}

==> tables/summarization.tex <==
\begin{table*}[t]
\centering
\scalebox{0.78}{
\begin{tabular}{lcccccc}
\toprule
                     & \multicolumn{3}{c}{CNN/DM} & \multicolumn{3}{c}{XSum} \\
                     & R1      & R2      & RL     & R1     & R2     & RL     \\
\midrule
BART-Base            & \cellcolor{black!20} $43.41_{\pm.06}$ & \cellcolor{black!20}$20.44_{\pm.03}$ & \cellcolor{black!20}$40.22_{\pm.03}$ & \cellcolor{black!20}$42.66_{\pm.04}$ & \cellcolor{black!20}$19.82_{\pm.01}$ & \cellcolor{black!20}$34.66_{\pm.06}$ \\
\ +Orig                & \cellcolor{blue!20}$43.20_{\pm.03}$ & \cellcolor{blue!20}$20.32_{\pm.04}$ & \cellcolor{blue!10}$40.03_{\pm.03}$ & $42.43_{\pm.07}$ & \cellcolor{blue!10}$19.68_{\pm.10}$ & \cellcolor{blue!10}$34.40_{\pm.08}$ \\
\ +Rand                & $42.71_{\pm.03}$ & $19.88_{\pm.01}$ & $39.53_{\pm.01}$ & $41.79_{\pm.10}$ & $19.13_{\pm.08}$ & $33.92_{\pm.08}$ \\
\ +SSM                 & \cellcolor{blue!10}$43.17_{\pm.08}$  & \cellcolor{blue!10}$20.26_{\pm.07}$ & \cellcolor{blue!10}$39.99_{\pm.09}$ & $42.43_{\pm.09}$  & $19.64_{\pm.13}$ & $34.50_{\pm.13}$        \\
\ +MaskFirst            & $43.09_{\pm.03}$ & $20.14_{\pm.03}$ & $39.92_{\pm.03}$ & $42.33_{\pm.05}$ & $19.54_{\pm.03}$ & $34.33_{\pm.03}$ \\
\ +MaskRandom          & \cellcolor{blue!30}$43.26_{\pm.06}$ & \cellcolor{blue!30}$20.32_{\pm.06}$ & \cellcolor{blue!30}$40.11_{\pm.05}$ & \cellcolor{blue!30}$42.61_{\pm.05}$ & \cellcolor{blue!30}$19.78_{\pm.05}$ & \cellcolor{blue!30}$34.60_{\pm.10}$ \\
\ +Supervised-CNN/DM   & \cellcolor{blue!20}$43.25_{\pm.11}$ & \cellcolor{blue!20}$20.31_{\pm.08}$ & \cellcolor{blue!10}$40.07_{\pm.09}$ & \cellcolor{blue!10}$42.45_{\pm.09}$ & $19.61_{\pm.06}$ & $34.42_{\pm.07}$ \\
\ +Meta-learned-CNN/DM & \cellcolor{blue!10}$42.83_{\pm.29}$ & $19.95_{\pm.26}$ & $39.62_{\pm.30}$ & $42.38_{\pm.03}$ & $19.63_{\pm.03}$ & \cellcolor{blue!10}$34.41_{\pm.06}$ \\
\ +Meta-learned-XSum   & $43.12_{\pm.04}$ & $20.20_{\pm.06}$ & $39.94_{\pm.04}$ & $42.28_{\pm.05}$ & $19.58_{\pm.05}$ & $34.36_{\pm.03}$ \\
\bottomrule
\end{tabular}
}
\caption{Full Results on Summarization Tasks.}\label{tab:summarization}

\end{table*} 

==> tables/summarization_simplified.tex <==
\begin{table}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{lcccccc}
\toprule
                     & CNN/DM & XSum \\
                    %  & R1      & R2      & RL     & R1     & R2     & RL     \\
\midrule
BART-Base            &  \cellcolor{black!20}$40.22_{\pm.03}$ & \cellcolor{black!20}$34.66_{\pm.06}$ \\
\ +Orig                & \cellcolor{blue!10}$40.03_{\pm.03}$ & \cellcolor{blue!10}$34.40_{\pm.08}$ \\
\ +Rand                & $39.53_{\pm.01}$ & $33.92_{\pm.08}$ \\
\ +SSM                 & \cellcolor{blue!10}$39.99_{\pm.09}$ & $34.50_{\pm.13}$        \\
\ +MaskFirstSentence   & $39.92_{\pm.03}$ & $34.33_{\pm.03}$ \\
\ +MaskRandomSentence  & \cellcolor{blue!30}$40.11_{\pm.05}$ & \cellcolor{blue!30}$34.60_{\pm.10}$ \\
\ +Supervised-CNN/DM   & \cellcolor{blue!10}$40.07_{\pm.09}$ & $34.42_{\pm.07}$ \\
\ +Meta-learned-CNN/DM & $39.62_{\pm.30}$ & \cellcolor{blue!10}$34.41_{\pm.06}$ \\
\ +Meta-learned-XSum   & $39.94_{\pm.04}$ & $34.36_{\pm.03}$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Rouge-L Performance of Abstractive Summarization Tasks.}. Full results that includes Rouge-1 and Rouge-2 can be found in the Appendix \ref{app:summ}.}\label{tab:summarization-simplified}
\vspace{-0.5cm}
\end{table} 
